Tell me more: Intent Fulfilment Framework for Enhancing User Experiences in Conversational XAI

The evolution of Explainable Artificial Intelligence (XAI) has emphasised the significance of meeting diverse user needs. The approaches to identifying and addressing these needs must also advance, recognising that explanation experiences are subjective, user-centred processes that interact with users towards a better understanding of AI decision-making. This paper delves into the interrelations in multi-faceted XAI and examines how different types of explanations collaboratively meet users' XAI needs. We introduce the Intent Fulfilment Framework (IFF) for creating explanation experiences. The novelty of this paper lies in recognising the importance of "follow-up" on explanations for obtaining clarity, verification and/or substitution. Moreover, the Explanation Experience Dialogue Model integrates the IFF and "Explanation Followups" to provide users with a conversational interface for exploring their explanation needs, thereby creating explanation experiences. Quantitative and qualitative findings from our comparative user study demonstrate the impact of the IFF in improving user engagement, the utility of the AI system and the overall user experience. Overall, we reinforce the principle that "one explanation does not fit all" to create explanation experiences that guide the complex interaction through conversation.

==> prelim.tex <==
\section{Preliminaries and Related Work}
\label{sec:prelim}

\begin{description}
\item [AI system] is a computational tool or entity designed to perform a task with the use of Artificial Intelligence. 
\item [Stakeholder] is an individual or group that has a vested interest or impact on the development, deployment, or outcomes of the AI system.  
\item [Explanation] refers to information that is offered by the AI system to a stakeholder as clarification, justification and/or evidence. 
\item [Explanation Target] is the specific aspect, feature, or element of an AI system's behaviour or output for which an explanation is sought by a stakeholder. 
\item [Intent] is the purpose, motivation or goal of a stakeholder for seeking explanations from the AI system.
\item [Explanation Technique/Explainer] is a method, algorithm, or approach employed to extract, generate, or present explanations.  
\item [Explanation Type] categorises the nature of information provided by explanations. Examples include factual explanations, counterfactuals and feature attributions. 
\item [Explanation Strategy] is a mapping between intents and techniques to address them. 
\item [Explanation Experience] is a session of interactions between a stakeholder with the AI system, articulating explanation
intents, receiving explanations and assessing their experience. 
\end{description}

\subsection{Multi-faceted XAI}
Taxonomies of Techniques, Types and Intents go here with their gaps. 
Gap: mapping between techniques and intents is often use case-specific. but there is an opportunity to create a general set of guidelines. 

One explanation does not fit all Taxonomy:~\cite{arya2019one}
 - not user-centred design - start with an intent
 - ignore simple explanations seek by the majority
 - no relationships between explanations

 
An important distinction between other taxonomies~\cite{arya2019one} and ours is that intents are mapped with explanation types instead of explainability techniques. 

\subsection{Conversational XAI}
Conversation is an upcoming medium for implementing interactive XAI, offering an alternative to graphical or text-based user interfaces~\cite{chromik2021human,madumal2019grounded,sokol2020one,malandri2023convxai}.


==> study_backup.tex <==
\section{Evaluation}
\label{sec:study}

We conduct a comparative user study to evaluate the impact of newly introduced dialogue types on intent fulfilment. 

\subsection{Study Applications}
\label{sec:app}

The study is based on the well-known loan approval use case. Three XAI researchers~(who had previous experience as loan applicants) curated the IFF for loan applicants as highlighted in bold black lines in Figure~\ref{fig:iff}. 
They selected 4 intents, 2 explanation targets and several explanation types for which the framework highlighted intent questions annotated with typology classifications. 
We configured two versions of the chatbot for comparison:
\begin{description}
\item \textbf{A)} For a given intent question, the chatbot only provides the default explanation; and
\item \textbf{B)} For a given intent question, after the default explanation, participant has the opportunity to follow up based on the secondary explanations available. Considering the participants are not domain or AI experts, the supplementary construct is automatically invoked with each explanation to provide textual annotations.
\end{description}
Both versions allow participants to ask multiple intent questions and receive multiple explanations. Each participant was assigned to one of the versions randomly creating the two comparative groups A and B. The study starts with a set of high-level study directions. Next, participants interact with their chatbot as loan applicants with no domain or AI expertise. A conversation is estimated to last for approximately 15 minutes. At the end, the chatbots prompt the participants to respond to an evaluation questionnaire and provide free-text feedback. 


\subsection{Recruitment}
This study involved 57 participants recruited via the Prolific platform. The criteria for recruitment included: fluency in the English language; qualification of (at least) an Undergraduate degree; and holding a single/joint bank account. 90 participants attempted the study within 7 days. We rejected 14 submissions from those who spent less than 1/3 of the estimated time and 19 did not complete the study.  Accordingly, 27 and 30 submissions were accepted for groups A and B. In each group, participants will be referred to as PA-1 and PB-1 etc. 

\subsection{Feedback Reliability}
Before analysis, we establish the reliability of the automatically collected feedback by examining the time elapsed during the interactions. The mean total time spent by groups A and B are TODO and 18.14 ± 10.63 minutes. The additional information provided by the supplementary dialogue constructs has significantly increased the interaction time of Group B. 
We exclude the following participants from the analysis following a critical review of their interaction times: PA-4 and PA-16 due to insufficient interaction time~($\leq$ 1/3 of the recommended time) and PB-25 due to inactivity~($\geq$ 4 times the recommended time). 
 
\subsection{Thematic analysis}

We performed a thematic analysis~\cite{saldana2021coding} of the free-text feedback from 25+29 participants from the two groups. The mean length of the responses was $122.89\pm 
37.65$ words. First, two independent codebooks were developed by four researcher ~(two per each group) using descriptive open coding that identifies emerging themes, patterns and concepts. Next, they reviewed independent codebooks and compared annotations to identify overlapping codes. They developed a shared codebook with consensus codes, definitions and supporting annotations representing both positive and negative sentiments. The shared codebook was reviewed to agree on 4 themes, each connected to $2-5$ codes, and these themes were subsequently named, defined and supported by relevant quote excerpts from the two groups. 
The themes identified were \textit{Presentation}, \textit{Comprehension}, \textit{Overall experience}, and \textit{Tool}. The first three encompass feedback that is not specific to the use cases, allowing for generalisable conclusions. All loan-approval use case-specific codes were grouped under the \textit{Tool} theme.

\subsubsection{Presentation}
This theme encapsulates the impressions of the participants regarding the quality and detail of the content presented.
In Group A the majority expressed the need for improvements in presentation. The feedback was distributed across different content entities such as the loan application, intent questions and explanations. The use of technical jargon and the tabular format of data affected the user experience.
\begin{quote}
\textit{``I do not know many words used by the bot, including “instance”, “test instance”, “rejected”, “0”, “1”, and many shortened names like int\_rate and verification\_status.''}(PA-7)
\end{quote}
Group B provided generally positive feedback regarding the content presentation. They understood the necessity for additional information provided by the ``Supplementary'' construct: \textit{``I found some of the explanations quite detailed and in some cases too detailed- but saying that I can see how this would be helpful.''} (PB-27). Participants from both groups provided suggestions to improve the presentation: PB-1 suggested breaking down the information into smaller chat bubbles; PA-5 suggested visually organising intent questions by their intent; and P23 suggested improving the responsiveness of the chatbot to different screen sizes.

\subsubsection{Comprehension}
This theme identifies how the content representations contributed to the participant’s understanding. 
Many from Group A found the content in charts or table formats was not easy to digest unless they had some domain and AI expertise: \textit{``I think some signposting or just brief explanations of the terms and models and used would have been useful''} (PA-25). Some participants expressed an expectation mismatch, noting that the content, specifically explanations were not adequately tailored to their knowledge level: \textit{``...information was non-intuitive and difficult to understand, as well as likely being quite daunting to users who are less technologically literate''}. (PA-9).
Additional information provided by the supplementary constructs addressed this exact shortcoming.
\begin{quote}
\textit{``The answers were not only detailed in the words ... but also bot used graphs, figures and images to explain the statistics behind the reasoning...''} (PB-19).   
\end{quote}
Many commented on how the detailed explanations improved their overall understanding of the domain and in AI: \textit{``I found the explanation complete enough to understand its applications and how to use it.''} (PB-7). They also indicated that the extra information helped close the gaps in domain knowledge: \textit{``...I didn’t expect that much level of detail, although it was needed because of my lack of knowledge surrounding the subject.''} (PB-19). Some reiterated their interpretation of the explanations and relationships between them, which helped us in validating their understanding: \textit{``LIME visualizes how qualities influence decisions, whereas Counterfactual depicts attribute alterations that potentially change outcomes.''} (PB-20).


\subsubsection{Overall experience} A prominent theme that emerged from participants’ feedback was their overall user experience while interacting with the chatbot.
The close-ended nature of the conversation received mixed reactions: \textit{``... I liked that it prompted you to ask questions and provided you with options of what to ask, however, it would have been better if I was able to type questions that I wanted to learn about''}. (PA-12). Some participants perceived that the content had not been tailored to a conversational experience. 
Generally more positive feedback was received from Group B. 
\begin{quote}
\textit{``My experience using the chatbot was good, it went smoothly.''} (PB-6)
\end{quote}
Participants highlighted features of the chatbot that contributed to a positive user experience. Provenance contributed to establishing trust in the system: \textit{``I appreciate that it also explained where it is getting its information from.''} (PB-1). The real-time interactions fostered a sense of transparency that may be lacking in an offline interaction where the decisions/explanations are already been made: \textit{``I felt that the explanations were refreshingly transparent in how it feeds user data into an algorithm to generate the decision.''} (PB-8), \textit{``...from a transparency perspective, the level of detail provided is so high as it will give people an unbiased understanding of why they have been accepted or rejected and actions they can take.''} (PB-26).


\subsubsection*{\textbf{Support}}
This theme encapsulates use-case-specific codes such as ``purpose of the loan approval chatbot'', ``utility of the chatbot in the real world'' and ``utility within the standard loan approval process''.  Participants expressed the purpose of the chatbot as follows: 
\begin{quote}
\textit{``“the bot was able to provide detailed evidence of the explanation behind the process of creating an answer which makes it more trustworthy''}(PA-15)
\end{quote}
Several Group A participants indicated that they failed to understand the purpose of the chatbot through interaction leading to a lack of trust: ``\textit{... there was no clear explanation about what was going on.}'' (PA-1). 
In contrast, Group B clearly understood the purpose of the tool and found it educational: \textit{``... the explanation experience was so thorough, that I feel as though I've gained a solid understanding of how the loan application process typically works. ''} (PB-15). 
They also provided validating evidence that a Loan Approval AI system has real-world significance and consequences in terms of explainability of AI decisions: \textit{``This helps users gain insights into the factors that influence decisions, which is especially useful when dealing with critical matters like loan approvals''} (PB-23). This led to them envisioning the utility of the chatbot as a tool for lenders: \textit{``This tool would help any banking institution or lenders in providing a clear method for approving loans by applicants''} (PB-2) as well as a self-assessment tool for applicants: \textit{``This gives more options for self-assessments, meaning less involvement needed from financial companies.''} (PB-30). 


\subsection{Quantitative Evaluation}
The responses to the evaluation questionnaire yielded quantitative evidence. The 7 questions were selected from the Explanation Satisfaction Scale and Explanation Goodness Checklist~\cite{hoffman2018metrics} and participants responded on a 5-step Likert scale. While exact questions were use-case specific, we hypothesise that the overarching difference in the sentiment between the two groups is representative of the user experience. Figure~\ref{fig:eval-responses} plots the response count of Group B over Group A. Overall, Group B demonstrated an overwhelmingly positive experience evidenced by the increase in positive responses and a decrease in negative/neutral responses.


\begin{figure*}[!ht]
\centering
\includegraphics[width=.9\textwidth]{evalq}
\caption{Evaluation Questionnaire Response Difference of Group B over Group A}
\label{fig:eval-responses}
\end{figure*}

\begin{figure*}[!ht]
\centering
\includegraphics[width=.9\textwidth]{evalq-diff}
\caption{Evaluation Questionnaire Response Difference of Group B over Group A}
\label{fig:eval-responses}
\end{figure*}



\subsection{Evaluation Outcomes}

\subsubsection{Intent Fulfilment}
Both groups executed all intents comparably. But Group B understood the explanations and overall more happy.

\subsubsection{Overall User Experience}
We argue the overall enhanced experience of Group B is significantly influenced by the additional information made available through the new dialogue constructs. 

In general explanations on their own are not enough - need natural language descriptions/summaries, alternative visualisations, to improve understanding. LLMs MM-LLMs can be utilised here.  - clear need for supplementary construct. others to be validated. 
